GreedyNASv2: Greedier Search with a Greedy Path Filter

Training a good supernet in one-shot NAS methods is difficult since the search space is usually considerably huge (e.g., $13^{21}$). In order to enhance the supernet's evaluation ability, one greedy strategy is to sample good paths, and let the supernet lean towards the good ones and ease its evaluation burden as a result. However, in practice the search can be still quite inefficient since the identification of good paths is not accurate enough and sampled paths still scatter around the whole search space. In this paper, we leverage an explicit path filter to capture the characteristics of paths and directly filter those weak ones, so that the search can be thus implemented on the shrunk space more greedily and efficiently. Concretely, based on the fact that good paths are much less than the weak ones in the space, we argue that the label of "weak paths" will be more confident and reliable than that of "good paths" in multi-path sampling. In this way, we thus cast the training of path filter in the positive and unlabeled (PU) learning paradigm, and also encourage a \textit{path embedding} as better path/operation representation to enhance the identification capacity of the learned filter. By dint of this embedding, we can further shrink the search space by aggregating similar operations with similar embeddings, and the search can be more efficient and accurate. Extensive experiments validate the effectiveness of the proposed method GreedyNASv2. For example, our obtained GreedyNASv2-L achieves $81.1\%$ Top-1 accuracy on ImageNet dataset, significantly outperforming the ResNet-50 strong baselines.

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/algs/train_supernet.tex <==
\begin{algorithm}[t]
	\caption{Training supernet with a greedy path filter.}
	\label{alg:train_supernet}
	
	\begin{algorithmic}[1]
	    \REQUIRE{Supernet $\N$, path filter $\P$, max training iteration $N$, train dataset $\D_{tr}$, small validation dataset $\D_{val}$, predictor update interval $t$, number of evaluation paths $m$, weak path prior $q$, merge operation threshold $\eta$.}
	    %\ENSURE{x}
	    \FOR{$i=1,...,N$}
	        \STATE $\bm{a}_i\sim U(\N)$ ;\hfill$\triangleright$ \gray{sample one path uniformly}
	        \WHILE{is\_weak\_arch($\P$, $\bm{a}_i)$}
	            \STATE $\bm{a}_i\sim U(\N)$ ;
	        \ENDWHILE
	        \STATE train($\N$, $\bm{a}_i$, $\D_{tr}$); \hfill$\triangleright$ \gray{train for one iteration}
	        \IF{$i$ \% $t$ = 0}
	            \STATE sample $m$ paths $\A=\{\bm{a}_j\}_{j=1}^m$ i.i.d \wrt $\bm{a}_j\sim U(\N)$ ;
	            \STATE $\bm{s}=\{\mbox{evaluate}(\N, \bm{a}_j, \D_{val})\}^m_{j=1}$ ;
	            \STATE $\A_{weak} = \mbox{last}(\bm{s}, q)$; \hfill$\triangleright$ \gray{get last $q$ percentile paths}
	            \STATE train predictor $\P$ with $\A_{weak}$ ;
	            \STATE merge operations according to Section~\ref{sec:op_shrinkage};
	        \ENDIF
	    \ENDFOR
	    %\RETURN x
	\end{algorithmic}
\end{algorithm}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/document.tex <==
%%%%%%%%% TITLE - PLEASE UPDATE
\title{GreedyNASv2: Greedier Search with a Greedy Path Filter}

\author{%
	Tao Huang${}^{1,2}$ \quad Shan You$^{1,3}$\thanks{Correspondence to: Shan You $<$\texttt{youshan@sensetime.com}$>$.}  \quad Fei Wang$^4$  
	\\
	Chen Qian$^1$ \quad Changshui Zhang$^{3}$ \quad Xiaogang Wang$^{1,5}$ \quad Chang Xu$^2$\\
	%~\\
	\normalsize $^1$SenseTime Research \quad
	\normalsize $^2$School of Computer Science, Faculty of Engineering, The University of Sydney \\
	\normalsize $^3$Department of Automation, Tsinghua University,
    \normalsize Institute for Artificial Intelligence, Tsinghua University (THUAI), \\
    \normalsize Beijing National Research Center for Information Science and Technology (BNRist)\\
	\normalsize $^4$University of Science and Technology of China \quad $^5$The Chinese University of Hong Kong\\ 
}

\begin{comment}
\author{First Author\\
Institution1\\
Institution1 address\\
{\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Second Author\\
Institution2\\
First line of institution2 address\\
{\tt\small secondauthor@i2.org}
}
\end{comment}
\maketitle

%%%%%%%%% ABSTRACT
\begin{abstract}
Training a good supernet in one-shot NAS methods is difficult since the search space is usually considerably huge (\eg, $13^{21}$). In order to enhance the supernet's evaluation ability, one greedy strategy is to sample good paths, and let the supernet lean towards the good ones and ease its evaluation burden as a result. However, in practice the search can be still quite inefficient since the identification of good paths is not accurate enough and sampled paths still scatter around the whole search space. In this paper, we leverage an explicit path filter to capture the characteristics of paths and directly filter those weak ones, so that the search can be thus implemented on the shrunk space more greedily and efficiently. Concretely, based on the fact that good paths are much less than the weak ones in the space, we argue that the label of ``weak paths" will be more confident and reliable than that of ``good paths" in multi-path sampling. In this way, we thus cast the training of path filter in the positive and unlabeled (PU) learning paradigm, and also encourage a \textit{path embedding} as better path/operation representation to enhance the identification capacity of the learned filter. By dint of this embedding, we can further shrink the search space by aggregating similar operations with similar embeddings, and the search can be more efficient and accurate. Extensive experiments validate the effectiveness of the proposed method GreedyNASv2. For example, our obtained GreedyNASv2-L achieves $81.1\%$ Top-1 accuracy on ImageNet dataset, significantly outperforming the ResNet-50 strong baselines.
\end{abstract}

%%%%%%%%% BODY TEXT
\section{Introduction} \label{sec:intro}

Neural architecture search (NAS) aims to boost the performance of deep learning by seeking an optimal architecture in the given space, and it has achieved significant improvements in the sight of applications, such as image classification \cite{tan2019efficientnet,guo2020single,you2020greedynas,su2021vision,yang2020ista} and object detection \cite{chen2019detnas,guo2020hit}. One-shot NAS \cite{guo2020single,you2020greedynas,su2021prioritized,yang2021towards,huang2020explicitly,su2021bcnet,su2020locally} stands out from the literature of NAS for the sake of its decent searching efficiency. Instead of exhaustively training each possible architecture, one-shot NAS fulfills the searching in an only one-shot trial, where a supernet is leveraged to embody all candidate architectures (\ie, paths). Each path can be parameterized by the corresponding weights within the supernet, and thus gets trained, evaluated, and ranked. 
Typical uniform sampling (SPOS) \cite{guo2020single} is usually adopted to train the supernet because of the feasible single-path memory consumption and being friendly to large-scale datasets. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/figure1.pdf}
    %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
    \vspace{-6mm}
    \caption{Performance of searched architectures \wrt different scales of search space. Left: retraining accuracies of models searched by GreedyNASv2 and baselines. Right: validation accuracies of searched models on supernets.}
    \label{fig:figure1}
    \vspace{-4mm}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/overview.pdf}
    \caption{Left: the architecture of our path filter. Right: diagram of supernet training in GreedyNASv2. In GreedyNASv2, we adopt a path filter to filter weak paths from the uniformly-sampled paths, and the remained potentially-good paths are then used for optimization. The path filter is trained using weak paths identified by a validation set and unlabeled paths.}
    \label{fig:figure2}
    \vspace{-4mm}
\end{figure*}

The architecture search space in NAS could be considerably huge (\eg, $13^{21}$). Equally treating different paths and uniformly sampling them from the supernet could lead to inappropriate training of the supernet, as the weak paths would disturb the highly-shared weights. Various sampling strategies have thus been proposed to address this issue, such as fair sampling \cite{chu2021fairnas} and Monte-Carlo tree search \cite{su2021prioritized}. We are particularly interested in the strategy of multi-path sampling with rejection by GreedyNAS \cite{you2020greedynas}, which identifies good paths from weak paths and then only greedily updates those good ones; it is easy to implement and more suitable for large search spaces among these methods. Working on the whole search space, GreedyNAS has to safely allocate only a medium level of partition of good paths (\eg, only 5 out of 10) to ensure a high probability of sampled paths being good. But the search will become infeasible and limited if the search space grows larger with more operation choices. Besides, GreedyNAS needs to maintain a candidate pool to recycle paths, which limits the number of stored paths, and many \textit{elite paths} could be missed. 

In this paper, we propose GreedyNASv2 to power the multi-path sampler with explicit search space shrinkage for one-shot NAS, which targets on a greedier search space with an tiny (\eg, only 1\%) proportion of paths treated as ``good paths''. Since good paths are usually much less than weak paths, the probability of picking out a good path by a multi-path sampler could be smaller than that of sampling weak paths. If weak paths can be captured with confidence, we can easily screen them out from the searching space and execute a greedier search on the shrunk space. By doing so, the supernet only needs to focus on evaluating those not too bad paths (potentially-good paths), which benefits the overall searching performance and efficiency simultaneously.

The key is then to learn a path filter to identify those weak paths from the entire architecture search space. Though it is hard to find a good path, we can have high confidence about weak paths in the multi-path sampling. These identified weak paths with confidence can be regarded as positive examples to be thrown away. As a precaution, the remaining paths in the search space are taken as unlabeled examples, as they may contain both weak paths (positive examples to be thrown away) and good paths (negative examples not to be thrown away). The learning of this path filter can thus be formulated as the Positive-Unlabeled (PU) learning problem \cite{letouzey2000learning, elkan2008learning}. Once the path filter has been well trained,  a given new path can be efficiently predicted to specify whether it is weak or not. A path embedding is also learned with the path filter to encode the path as a better path representation. Since the path embedding is learned in the weak/good sense, if two operations have similar embeddings, it means that both operations have similar or even the same impact on discriminating paths, and they can be thus merged. This enables a greedy shrinkage of operations, which is expected to work together with the path shrinkage to boost the searching performance and efficiency further. 

We conduct extensive experiments on ImageNet dataset to validate the effectiveness of our proposed GreedyNASv2. Compared to the baseline methods SPOS and GreedyNAS, our proposed method achieves better performance with less search cost. To further investigate our superiority, we even search on a larger space, which has $\sim 10^4\times$ architectures compared to the commonly-used MobileNetV2-SE search space, and the results show that our searched model outperforms state-of-the-art NAS models. The performance on different scales of search spaces are illustrated in Figure~\ref{fig:figure1}. Besides, we also compare the searching performance on a recent benchmark NAS-Bench-Macro \cite{su2021prioritized} for one-shot NAS. Ablation studies show that our GreedyNASv2 effectively samples better architectures than uniform sampling and the multi-path sampler in GreedyNAS.

\section{Related Work}


\subsection{NAS with search space shrinkage}
\textbf{Path-level shrinkage.} To obtain a path-level shrinkage on search space, GreedyNAS~\cite{you2020greedynas} proposes a candidate pool to store those evaluated good paths and samples from it using an exploration-exploitation strategy. MCT-NAS~\cite{su2021prioritized} proposes to sample architectures with the guidance of Monte-Carlo tree search; hence the good paths can be sampled with better exploration and exploitation balance. However, the limited size (\eg, 1000) of candidate pool in GreedyNAS is too aggressive to train the elite paths with enough diversity, and the exponentially-increased Monte-Carlo tree makes the MCT-NAS difficult to scale to larger search spaces.

\textbf{Operation-level shrinkage.} Operation-level shrinkage is also an effective way to reduce both training parameters and the size of search space. Some methods~\cite{hu2020angle,shen2020bs} design importance metrics to identify the good operations and drop the weak ones. For example, ABS~\cite{hu2020angle} measures the importance of each operation using the angle between its trained weights and initialized weights; BS-NAS~\cite{shen2020bs} proposes a channel-level importance metric by measuring a number of architectures on the validation dataset. However, these methods only consider operation-level statistics, while for each specific architecture, the preferences of operations may be different. On the other hand, NSENet~\cite{ci2021evolving} proposes to learn the importance using additional learnable indicators after each operation, which is learned by simulating the gradients of binary-selected architectures. However, this simulation of gradients introduces approximation errors and also increases memory consumption. 

In this paper, we perform both path-level and operation-level shrinkage using a path filter. The path filter is constructed by a binary classifier, which efficiently filters the weak paths and generalizes well to the whole search space; hence we can filter the weak paths more greedily. Furthermore, we can perform operation-level shrinkage without extra costs by measuring the learned operation embeddings in the path filter. This operation merging strategy holds naturally since the operations with similar embeddings would have similar predictions and thus similar performance.

\subsection{Positive-unlabeled learning}
Positive-Unlabeled (PU) classification is a problem of training a binary classifier from only positive and unlabeled data \cite{letouzey2000learning, elkan2008learning}. 
\begin{comment}
In NAS, it only has a very small portion of good paths in the search space, so that we have a small confidence on labeling good paths while the confidence on weak paths is fairly large. This naturally formulates a PU problem: \textit{with only labeled reliable weak paths and unlabeled paths, how can we learn a predictor to distinguish the good and weak architectures?} Luckily, this problem is widely discussed in PU learning and many effective methods~\cite{du2015convex,kiryo2017positive,chen2020vpu} are proposed to train a good binary classifier. 
\end{comment}
Many effective methods~\cite{du2015convex,kiryo2017positive,chen2020vpu} are proposed to train a good binary classifier in PU learning. Specifically, uPU~\cite{du2015convex} rewrites the classification risk in terms of the distributions over positive and unlabeled samples, and obtains an unbiased estimator of the risk without negative samples. To overcome the overfitting problem in uPU, a non-negative risk estimator is proposed in nnPU\cite{kiryo2017positive}. One recent approach VPU~\cite{chen2020vpu} proposes a variational principle for PU learning without involving class prior estimation or any other intermediate estimation problems. In this paper, we implement VPU to learn our path filter.



\section{Revisiting Multi-path Sampler}
In single path one-shot NAS~\cite{guo2020single, you2020greedynas, su2021prioritized}, the search space is treated as an over-parameterized supernet $\N$, in which the searching layers are stacked sequentially, and each layer is required to select one operation from candidate operations. Assume the supernet has $L$ layers and $N$ candidate operations $\O=\{o_i\}, \forall i = 1,2,...,N$, then each architecture can be represented by a tuple with size $L$, \ie, $\bm{a}=(o^{(1)}, o^{(2)}, ..., o^{(L)})$, where $o^{(j)} \in \O$, $\forall j = 1,2,...,L$. As a result, the search space $\A$ is of size $|\A| = N^L$. With a pre-defined supernet, the NAS procedure is split into two stages: supernet training and search. During training, the supernet is optimized by alternately sampling paths and updating their corresponding weights. Thereafter, the optimal path can be determined as the one with the highest accuracy on a hold-out validation set. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/confidence.pdf}
    \vspace{-6mm}
    \caption{Confidence $\mathbb{P}$ ($\mathbb{Q}$) of sampling at least $k$ good (weak) paths out of $m=10$ paths with proportion $p$ of good paths.}
    \vspace{-2mm}
    \label{fig:confidence}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/merge.pdf}
    \caption{Overview of the proposed operation shrinkage method. We evaluate the cosine similarities of operation pairs in each layer using the learned operation embeddings. Then, we merge the similar operation pair to one operation with smaller FLOPs.}
    \label{fig:merge}
\end{figure*}


Although the supernet shares weights with all architectures, it still has $\sim N\times$ parameters than a common path. For example, the benchmark MobileNetV2-SE search space has $13$ operations and $46$M parameters for supernet, while a path only has $\sim 5$M parameters. With such a large supernet, it is harsh to optimize all the architectures well and evaluate them accurately. Therefore, instead of sampling paths uniformly \cite{guo2020single}, GreedyNAS~\cite{you2020greedynas} proposes a multi-path sampling with rejection to greedily sample those potentially-good paths; hence the training efficiency and performance can be boosted.

\subsection{Frustrating sampling good paths}

In the multi-path sampler, $m$ paths are sampled at once, then evaluated and ranked by a small validation set. According to the Theorem~\ref{theorem1} below, we can thus safely treat the Top-$k$ paths as good ones, and train the supernet greedily by just updating these $k$ paths. 
\input{theorem1.tex}
To ensure a high confidence $\mathbb{P}$ of sampling good paths, GreedyNAS only has to assume a medium level of good path proportion (\ie, large $p$). For example, $\mathbb{P}$ comes to $83.38\%$ with $p=0.6$ when we leave $k=5$ paths as good from the sampled $m=10$ paths.

However, this is not enough. Since we target at the optimal architecture, the candidate \textit{elite} paths are supposed to be way less than the weak ones, which means that $p\ll 0.5$ holds naturally, and thus we can have an actually shrunk space to boost the searching. Frustratingly, the confidence will degrade according; for example, with $p=0.1$, the previous confidence $\mathbb{P}$ will be only $0.16\%$. Though GreedyNAS leverages a candidate pool to recycle paths, many \textit{elite paths} could be missed since it heavily relies on the limited number of stored paths (\eg, 1000). 


\subsection{Turning tables with weak paths}
Sampling good paths is frustratingly ineffective in a more greedy space since the confidence collapses as a failure. In contrast, since the good prior $p$ is low, the search space will be glutted with weak paths, and the probability of sampling a weak path $q:= 1-p$ is thus large accordingly. Similarly, based on Theorem \ref{theorem1}, in multi-path sampling the confidence of sampled weak paths goes even larger, denoted as $\mathbb{Q}:= \sum_{j=k}^m\mathbb{C}_m^j q^j (1-q)^{m-j}$. For example, with $q=0.9$ ($p=0.1$), the probability of sampling at least $5$ weak paths out of $10$ is very high ($\mathbb{Q}=99.99\%$). See Figure \ref{fig:confidence} for more details. 

Now the tables have been turned. If we can sample weak paths with high confidence, we can easily rule them out from the entire search space and implement a more greedily searching on the shrunk space, thus boosting the searching performance as well. Then the question goes to: how can we leverage the sampled weak paths to identify a shrunk space composed of good paths? Intuitively, we encourage learning a path filter to encode the characteristics of sampled weak paths and identify the label of a given new path.

Nevertheless, during multi-path sampling, we only have confidence about weak paths, \textit{can we still learn a discriminative path filter as a decent binary classifier to predict labels of paths?} The answer is affirmative; in the sequel, we will cast the learning as a typical Positive and Unlabeled (PU) problem. 

\section{Greedier Sampling with a Path Filter}
\begin{comment}
In this paper, we propose to achieve greedier sampling with a path filter, which is a binary classifier to predict whether a path is weak or not. We greedily filter those paths with weak predictions and sample the remained good ones for optimization. Since the path filter predicts paths much faster than evaluating paths in multi-path sampling, we can efficiently predict a batch of paths one time and filter a large percentage of paths for greedy training.
\end{comment}

After multi-path sampling, we now have confident weak paths; nevertheless, remaining paths are difficult to specify whether they are weak or good, since the corresponding confidence will be low. As a precaution, we regard the remaining paths (together with unsampled paths) as unlabeled examples, as they may contain both weak and good paths. 

\subsection{Learning path filter as PU prediction}
Here we want to learn a path filter with the identified weak paths (positive examples) and remaining paths (unlabeled examples). Formally, let us first consider a binary classification problem where the architectures $\a\in\A$ and class labels $y\in\{-1,+1\}$ are distributed according to a joint distribution $\mathbb{D}(\a,y)$, and the paths with positive label $+1$ denote weak paths to be discarded. In GreedyNASv2, we have positive dataset $\P = \{\a_1, ..., \a_M\}$ and unlabeled dataset $\U = \{\a_{M+1},...,\a_{N}\}$ sampled from the search space. The learning of path filter is thus cast as a Positive and Unlabeled (PU) learning problem, where a binary predictor $\Phi$ is learned based on $\P$ and $\U$ so that the class labels of unseen architectures can be accurately predicted.


As an introduction of PU learning, we first investigate the expected risk (classification loss) on the whole dataset of the commonly supervised learning (PN learning) as 
\begin{equation} \label{eq:cls_risk}
    R(\Phi) = \pi_\P\mathbb{E}_\P[l_{+}(\Phi(\a))] + (1-\pi_\P)\mathbb{E}_\N[l_{-}(\Phi(\a))] ,
\end{equation}
where $\pi_\P = \mathbb{P}(y=+1)$ denotes the \textit{class prior} of positive data, $\N$ refers to negative dataset, and $l_+$ and $l_-$ denote classification losses with
\begin{align}
    \begin{split}
        \mathbb{E}_{\mathcal{P}}[l_+(\Phi(\bm{a}))] &= \frac1{|\P|} \sum_{\a\in\P} l(\Phi(\bm{a}),+1) ,\\
        \mathbb{E}_{\mathcal{N}}[l_-(\Phi(\bm{a}))] &= \frac1{|\N|} \sum_{\a\in\N} l(\Phi(\bm{a}),-1),
    \end{split}
\end{align}
which are the expectations of $l_+(\Phi(\bm{a}))$ on the positive dataset $\mathcal{P}$ and $l_-(\Phi(\bm{a}))$ on the negative dataset $\mathcal{N}$.


Nevertheless, the negative dataset $\N$ is unavailable in our PU learning setting. To train the model with positive and unlabeled data, the classical method uPU~\cite{du2015convex} encourages an unbiased formulation to the PN learning by rewriting the expectation of negative classification loss $\mathbb{E}_{\mathcal{N}}[l_-(\Phi(\bm{a}))]$ to 
%, we can rewrite the risk over the negative class-conditional distribution, \ie, 
\begin{equation} \label{eq:unbiased_negative}
    (1-\pi_\P)\mathbb{E}_\N[l_{-}(\Phi(\a))] = \mathbb{E}_\U[l_{-}(\Phi(\a))] - \pi_\P\mathbb{E}_\P[l_{-}(\Phi(\a))] ,
\end{equation}
%Based on Eq.(\ref{eq:unbiased_negative}), the classical method uPU~\cite{du2015convex} proposes an effective solution to PU learning by introducing the unbiased risk estimator
and thus Eq.(\ref{eq:cls_risk}) can be adapted to
\begin{equation}
    R(\Phi) = \pi_\P\mathbb{E}_\P[l_{+}(\Phi(\a))-l_{-}(\Phi(\a))] + \mathbb{E}_\U[l_{-}(\Phi(\a))] ,
\end{equation}
%which can achieve an unbiased estimation of the expected classification risk in Eq.(\ref{eq:cls_risk}). 

However, such a method easily leads to severe over-fitting, especially on deep neural classifiers. In our paper, to alleviate the above weakness, we leverage the learning objective in VPU~\cite{chen2020vpu}, which proposes a variational loss to approximate the ideal classifier through an upper-bound of Eq.(\ref{eq:cls_risk}), \ie, 
\begin{align}
    \label{eq:vpu}
    \begin{split}
        R(\Phi) &= \mbox{log}\mathbb{E}_\U[\Phi(\a)] - \mathbb{E}_{\P}[\mbox{log}\Phi(\a)] \\
        %&= \mbox{log}\frac{\sum_{\a\in\mathcal{B}_\U}\Phi(\a)}{B} - \frac{\sum_{\a\in\mathcal{B}_\P}\mbox{log}\Phi(\a)}{B} ,
    \end{split}
\end{align}
where mini-batches $\mathcal{B}_\U$ and $\mathcal{B}_\P$ are sampled from $\U$ and $\P$ with size $B$. By minimizing Eq.(\ref{eq:vpu}), we can obtain an effective binary classifier to distinguish good and weak paths.

\textbf{Train path filter with multi-path sampling.} We first construct a neural network as our path filter (binary classifier), which will be trained using PU learning. For the network structure, we follow a simple \textit{Embedding-RNN} pipeline as the previous work~\cite{zoph2016neural}. Concretely, as illustrated in Figure~\ref{fig:figure2} left, we use randomly initialized embeddings $\bm{E}\in \mathbb{R}^{L\times N \times H}$ to represent operations in the search space, where $L$, $N$, and $H$ are numbers of layers, candidate operations, and hidden dimensions, respectively, hence each operation in each layer is associated with an independent embedding. For example, the embedding of $j$-th operation $o_{j}^{(i)}$ in layer $i$ can be represented as $\bm{E}_{i,j}$ . For an input architecture $\bm{a} = (o^{(1)}, o^{(2)}, ..., o^{(L)})$, the predictor first encodes it through operation embedding $\bm{E}$ to get the hidden states $\bm{A}$ of the selected operations, where $\bm{A} \in \mathbb{R}^{L\times H}$. Then we use a bi-directional LSTM to get the feature $\bm{f}_a \in \mathbb{R}^{H}$ of the architecture. Finally, the architecture feature $\bm{f}_a$ is fed into a binary classifier (two-layer perceptions with intermediate ReLU activation) to obtain the prediction.

Following the multi-path sampling strategy in GreedyNAS, each time we train the path filter, we randomly sample $m$ paths and evaluate them using the loss on a small validation set, which contains $1000$ images sampled from the validation set. We sort those sampled paths with their losses in ascending order, and label the last $p$ percentage of paths as ``weak paths'' to build the positive dataset $\P$, while the unlabeled dataset $\U$ is constructed by uniformly sampling $10\times p\times m$ paths from the search space. With the learning objective in Eq.(\ref{eq:vpu}), we train the path filter with datasets $\P$ and $\U$ every $t$ epochs in the training of supernet to ensure its accuracy. Once the path filter is trained, it can be used to predict a batch of uniformly-sampled paths, and filter those paths with positive labels, and the remained paths are treated as the potentially-good paths and used in optimization.

\textbf{Stopping principle via path predictions.} In training, if the supernet is trained well, the rankings of paths tend to be steady; hence GreedyNAS proposes an early stopping principle by measuring the \textit{steadiness} of the candidate pool. We now propose a more accurate way by predicting more paths using the learned path filters, \ie, 
\begin{equation}
    u := \frac{\sum_{\bm{a}_i\in\A_r}\1_{\Phi_t(\bm{a}_i)=\Phi_{t-1}(\bm{a}_i)}}{M} > \beta,
\end{equation}
where $\A_r$ is a set of $M$ randomly sampled paths, $\Phi_t$ denotes the learned path filter at iteration $t$. $u$ measures the proportion of the same predictions in the last two path filters, if $u>\beta$, we believe the supernet has been trained enough, and its training can be stopped accordingly. We set $N = 10^4$ and $\beta = 0.9$ in our experiments.

\textbf{Evolutionary search with path filter.} We adopt evolutionary algorithm (EA) NSGA-II~\cite{deb2002fast} to search architectures. Unlike SPOS~\cite{guo2020single} generates architectures randomly and GreedyNAS~\cite{you2020greedynas} only specifies an initial population, we use the learned path filter to filter the weak architectures generated by EA during the whole search, thus the search could be more efficient.

\input{algs/train_supernet.tex}
\input{tables/search_space.tex}

\subsection{Shrinking operations with learned embeddings} \label{sec:op_shrinkage}
The PU predictor distinguishes whether a path is good or bad using learned operation embeddings. If the embeddings of two operations $o_a^{(i)}$ and $o_b^{(i)}$ in layer $i$ are totally the same, it means that for all the architectures, replacing $o_a^{(i)}$ by $o_b^{(i)}$ would not affect the classification results and vice versa. As a result, if two operations act similarly, we can greedily merge them and keep the less-costly one (\eg, the one with smaller FLOPs).

Cosine similarity is a commonly-used metric to measure the similarity of two vectors. Given two vectors $\bm{x}$ and $\bm{y}$, their cosine similarity $S_c(\bm{x}, \bm{y})$ is represented as 
\begin{equation}
    S_c(\bm{x}, \bm{y}) = \frac{\bm{x}\cdot\bm{y}}{\|\bm{x}\|\cdot \|\bm{y}\|} = \frac{\sum_{i=1}^n x_iy_i}{\sqrt{\sum_{i=1}^n x_i^2}\sqrt{\sum_{i=1}^n y_i^2}} .
\end{equation}

After each time we train the predictor, we will measure the cosine similarities between different operations in each layer. If the similarity between two operations is less than a pre-defined threshold $s_{\text{thrd}}$, we then merge these two operations into one operation by keeping the one with smaller FLOPs and removing another one. 

Formally, for operations $\{o_1^{(i)}, o_2^{(i)}, ..., o_N^{(i)}\}$ in layer $i$, it has $\mathbb{C}_N^2$ combinations of pairs, we compute their cosine similarity between $o_j^{(i)}$ and $o_k^{(i)}$ using the learned embeddings, \ie,
\begin{equation}
    S_{j,k}^{(i)} = S_c(\bm{E}_{i,j}, \bm{E}_{i, k}) .
\end{equation}
For any layer $i\le L$ and operation pairs $o_j^{(i)}$ and $o_k^{(i)}$ ($j<k\le N$), we merge them into the one with less FLOPs when they satisfy $S_{j,k}^{(i)} > s_{\text{thrd}}$. After merging, the removed operations would never be sampled in training and search, thus reducing the training parameters in supernet. We set $s_{\text{thrd}} = 0.8$ in our experiments.

Our operation shrinkage method can significantly reduce the search space without additional evaluation steps. It can be naturally combined with the path-level shrinkage to perform a greedier search. The overall supernet training strategy is summarized in Algorithm~\ref{alg:train_supernet}.

\section{Experiments}
\subsection{Experimental setup}

\input{tables/nas_comparison.tex}
\input{tables/imagenet.tex}

\textbf{Search space.} As summarized in Table~\ref{tab:search_space}, for comparisons with baselines~\cite{you2020greedynas, su2021prioritized}, we first search on MobileNetV2-SE search space, which consists of Identity, MobileNetV2 block~\cite{sandler2018mobilenetv2}, and optional SE modules~\cite{hu2018squeeze}. To validate our superiority on larger search spaces, we extend the search space with MixConv~\cite{tan2019mixconv} block, namely, \textit{MobileNetV2-SE+MixConv}. Moreover, we set up an extremely-large search space~\textit{MobileNetV2-SE+MixConv+Shuffle}, which adds $4$ ShuffleNetV2 blocks~\cite{ma2018shufflenet} following SPOS~\cite{guo2020single}. %\blue{Since the computation of ResNet like structures is more efficient than mobile networks with depth-wise convolution on GPUs}, 
In order to validate the effectiveness of our method on larger networks, we also introduce a ResNet-like search space, which consists of the blocks in ResNet~\cite{he2016deep}, ResNeXt~\cite{xie2017aggregated}, and SENet~\cite{hu2018squeeze}. Details can be found in supplementary materials.

\textbf{Supernet.} We randomly sampled $50$k images from ILSVRC-2012~\cite{imagenet} train set to build our validation set, and the remains are used as the training set. We train the supernet with an SGD optimizer and a total batch size of $1024$, a cosine learning rate which decays $120$ epochs with an initial learning rate $0.12$ is adopted. In the first $20$ epochs of training, we sample architectures uniformly for warm-up, then train the path filter every $5$ epoch and use it to sample architectures. The weak path prior $q$ is increased from $0.5$ to $0.99$ in $90$ epochs.

\textbf{Path filter.} The path filter is constructed by an embedding with $128$ dimensions, followed by a bidirectional LSTM and two fully-connected layers with intermediate ReLU activation, all the hidden dimensions are set to $128$. We train the path filter for $3000$ iterations after every $5$ epoch of the supernet training, an Adam optimizer with batch size $1024$ and weight decay $5\times10^{-3}$ is adopted, the learning rate is set to $10^{-3}$.

\textbf{Search.} We use the learned path filter to help the evolutionary algorithm NSGA-II~\cite{deb2002fast} search architectures. The search number is set to $500$. 

\textbf{Retraining.} In retraining, we use the official ILSVRC-2012~\cite{imagenet} train set and report the accuracy on the original validation set. Following \cite{you2020greedynas, su2021prioritized}, we train the searched mobile architectures using a RMSProp optimizer with a batch size $96$ on each of $8$ GPU, a step learning rate scheduler which warmups for $3$ epochs then decays $0.97$ every $2.4$ epochs is adopted with initial value $0.048$. While for ResNet-like model, we train it using SGD optimizer with weight decay $10^{-4}$ and batch size $1536$, the initial learning rate is set to $0.6$ and decays for $240$ epochs with a cosine scheduler.
We use a data augmentation pipeline of Autoaugment~\cite{cubuk2019autoaugment}, random cropping, and clipping. We use a train and test image size of $224\times224$. Besides, an exponential moving average on weights is also adopted with a decay $0.9999$.

\subsection{Results on ImageNet}
\textbf{Comparisons with NAS methods.} We first compare our GreedyNASv2 with the baseline methods SPOS~\cite{guo2020single} and GreedyNAS~\cite{you2020greedynas} on \textit{MB-SE}, \textit{MB-SE+MixConv}, and \textit{MB-SE+MixConv+Shuffle} search spaces based on our implementations. We use a constraint of $330$M FLOPs and report the evaluation accuracies of the searched architectures on retraining and supernet in Table~\ref{tab:nas_comparison}. We can see that, on all sizes of search spaces, our GreedyNASv2 can obtain higher ACCs than the other two methods. Moreover, the performance of SPOS on medium and large spaces drops significantly, showing that it would be difficult for SPOS to train promising supernets on such huge spaces. While our GreedyNASv2 obtains similar performance, and even achieves the best performance on large space. We compare our obtained model \textit{GreedyNASv2-S} on \textit{MB-SE+MixConv+Shuffle} search space with state-of-the-art NAS methods in Table~\ref{tab:imagenet}.

\textbf{Search for larger networks.} To evaluate our generalization, we conduct search on a ResNet-style search space \textit{Res-50-SE}. As the results shown in Table~\ref{tab:imagenet}, our GreedyNASv2 achieves significant improvement compared to the baseline ResNet, ResNeXt, and SENet models. Note that we train our \textit{GreedyNASv2-L} with simple SGD optimizer and an additional Autoaugment~\cite{cubuk2019autoaugment} data pipeline. However, its performance still outperforms the state-of-the-art training strategies with more sophisticated optimization and strong data augmentation in TIMM ~\cite{wightman2021resnet}, which achieves 80.4\% ACC on ResNet-50.

\subsection{Results on NAS-Bench-Macro}
MCT-NAS~\cite{su2021prioritized} proposes a NAS benchmark named NAS-Bench-Macro for single path one-shot NAS methods, which consists of $6561$ architectures and their isolated evaluation results on CIFAR-10 dataset. We leverage this benchmark to validate the effectiveness of GreedyNASv2.

\textbf{Performance of path filter with ground-truth training data.} To validate the pure performance of our PU learning method, we conduct experiments to train the path filter with the ground-truth labels in the benchmark. Concretely, we split the architectures to $10\%$ of good paths and $90\%$ of weak paths according to their evaluation accuracies, then samples $1\%,10\%,50\%$, and $100\%$ data as a train set. We use the whole set to validate the classification performance of the learned path filter. We use precision and recall as evaluation metrics. We first train the path filter with our PU learning settings using only weak paths and randomly sampled unlabeled paths. For comparisons, we also adopt the PN learning (traditional supervised learning) by using both weak labels and good labels. As the results reported in Table~\ref{tab:nasbench}, the PU learning even achieves better performance than PN learning. This might be because paths are densely distributed in the space, an absolute threshold for partitioning ``P'' and ``N'' data might involve many uncertain paths, while the PU learning could handle this uncertainty well by treating unlabeled data more safely.

\input{tables/nas_benchmark.tex}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/percentile_rank.pdf}
    \vspace{-2mm}
    \caption{Histogram of percentile rank of sampled paths on NAS-Bench-Macro search space. The average percentile rank of \textit{uniform sampling}, \textit{GreedyNAS}, and \textit{GreedyNASv2} are $50.6\%$, $18.1\%$, and $6.4\%$, respectively.}
    \label{fig:percentile_rank}
    \vspace{-4mm}
\end{figure}


\textbf{Performance of path filter on supernet.} We also validate the performance of the path filter learned in supernet training. Unlike the previous experiment using the ground-truth labels, the labels in supernet training are generated by evaluating sampled architectures with a validation set; hence, they could have some noises. The learned path filter obtains $93.74\%$ precision and $98.21\%$ recall on the whole search space, comparing to the best performance of using ground-truth labels ($98.81\%$ precision and $98.62\%$ recall), the small decrease in precision is acceptable since our method only needs to greedily focus on a proportion of potentially-good paths instead of locating all the good ones.

\textbf{Average percentile ranks of the sampled architectures during training.} We collect the percentile ranks of the sampled architectures during training. As shown in Figure~\ref{fig:percentile_rank}, our method samples more paths with smaller percentile ranks compared to baselines, which means that our trained supernet is greedier towards those good paths.

\textbf{Correlation between validation and retraining accuracies.} Since GreedyNASv2 greedily filters out weak paths and focuses on the potential good paths, the correlation between validation accuracies on supernet and their retraining accuracies will be boosted in terms of those good paths identified by the path filter. We measure the rank correlations on those paths within top 10\% percentile ranks on NAS-Bench-Macro, and the Kendall's Tau of SPOS, GreedyNAS, and GreedyNASv2 are 23.9\%, 41.5\%, and 50.3\%, respectively. This indicates our effectiveness since discriminating among good paths are fairly challenging. 

\subsection{Ablation studies}

\textbf{Visualization of learned operation similarities.} As summarized in Figure~\ref{fig:sim} and Table~\ref{tab:merge_ops}, we visualize the learned operation similarities at the first searching layer of MB-SE supernet. It shows that the operations with the same kernel size are more likely to have similar embeddings. For \textit{ID} operation, it has negative similarities to all the other operations since it performs poorly on down-sampling layers. For the whole supernet, there are a total of $35$ ($\sim 13\%$) out of $13\times 21 = 273$ operations merged.

\input{tables/merge_ops.tex}

\section{Conclusion}
We propose GreedyNASv2, a NAS method with greedy path-level and operation-level shrinkage of search space. Unlike the previous works, our method achieves a greedier search with a greedy path filter, which is trained with highly-confident ``weak'' paths and unlabeled paths using positive-unlabeled (PU) learning. By dint of the learned embeddings in our path filter, we can further perform operation-level shrinkage by aggregating similar operations with similar embeddings, and the search can be more efficient and accurate. Extensive experiments show that our GreedyNASv2 achieves better performance compared to our baselines in various scales of search spaces. 

\section*{Acknowledgements}
This work was supported in part by the Australian Research Council under Project DP210101859 and the University of Sydney SOAR Prize.

%%%%%%%%% REFERENCES
{\small
\bibliographystyle{ieee_fullname}
\bibliography{main}
}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> GreedyNASv2_ Greedier Search with Greedy Path Filter/tables/correlation.tex <==
\begin{table}[h]
	\renewcommand\arraystretch{1.17}
	\setlength\tabcolsep{3mm}
	\centering
	%\begin{center}
	\caption{Rank correlations of the evaluation results of similar, dissimilar, and random pairs identified by the path filter on supernet.}
	\vspace{-2mm}
	\label{tab:correlation}
	\footnotesize
	%\normalsize
	\begin{tabular}{c|c|c|c}
		\Xhline{2\arrayrulewidth}
		\multirow{2}*{Pairs} & \multirow{2}*{Mean similarity} & \multicolumn{2}{c}{Rank correlation (\%)}\\
		\cline{3-4}
		~ & ~ & Spearman's & Kendall's Tau\\
		\hline
		similar & 0.9118 & \textbf{99.26} & \textbf{93.68}\\
		dissimilar & -0.2183 & 73.38 & 69.58\\
		random & 0.3412 & 83.62 & 78.31\\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	\vspace{-4mm}
	%\end{center}
\end{table}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/tables/imagenet.tex <==
\begin{table*}[t]
	\renewcommand\arraystretch{1.17}
	\setlength\tabcolsep{4.5mm}
	\centering
	%\begin{center}
	\caption{Comparisons of searched architectures with state-of-the-art NAS methods and handcraft models. Training epochs and search number are hyper-parameters in the training of supernet. We measure the training cost of supernet using 8 NVIDIA V100 GPUs. *: trained with the same strategy as \textit{GreedyNASv2-L}.}
	\vspace{-2mm}
	\label{tab:imagenet}
	\footnotesize
	%\normalsize
	\begin{tabular}{r|cccc|ccc}
		\Xhline{2\arrayrulewidth}
		\multirow{2}*{Methods} & Top-1 & Top-5 & FLOPs & Params & Training & Training cost & Search\\
		%\cline{6-8}
		~ & (\%) & (\%) & (M) & (M) & epochs & (GPU days) & number\\
		\hline
		\multicolumn{8}{c}{mobile search space}\\
		\hline
		MobileNetV2~\cite{sandler2018mobilenetv2} & 72.0 & 91.0 & 300 & 3.4 & - & - & -\\
		%MnasNet-A1 & 75.2 & 92.5 & 312 & 3.9 & - & 288 & -\\
		EfficientNet-B0~\cite{tan2019efficientnet} & 76.3 & 93.2 & 390 & 5.3 & - & - & - \\
		%ABS~\cite{hu2020angle} & 74.4 & - & 325 & - & 105 & - & -\\
		SPOS~\cite{guo2020single} & 74.7 & - & 328 & 3.4 & 120 & 12 & 1000 \\ 
		%BS-NAS-A~\cite{shen2020bs} & 75.9 & 92.8 & 465 & 4.9 & 240 & 10 & 1500 \\
		MCT-NAS-B~\cite{su2021prioritized} & 76.9 & 93.4 & 327 & 6.3 & 120 & 12 & 100 \\
		K-shot-NAS-B~\cite{su2021k} & 77.2 & 93.3 & 332 & 6.2 & 120 & 12 & 1000 \\
		NSENet~\cite{ci2021evolving} & 77.3 & - & 333 & 7.6 & 100 & 166.7 & 2100 \\
		GreedyNAS-B~\cite{you2020greedynas} & 76.8 & 93.0 & 324 & 5.2 & 46 & 7 & 1000 \\
		\textbf{GreedyNASv2-S} & \textbf{77.5} & 93.5 & 324 & 5.7 & 65 & 7 & 500\\
		\hline
		\multicolumn{8}{c}{ResNet search space}\\
		\hline
		ResNeXt-50~\cite{xie2017aggregated} & 77.8 & - & 4230 & 25.0 & - & - & -\\
		RegNetX-4.0GF~\cite{radosavovic2020designing} & 78.6 & - & 3964 & 22.1 & - & - & -\\
		ResNet-50$^*$~\cite{he2016deep} & 78.8 & 94.6 & 4089 & 25.6 & - & - & -\\
		SE-ResNeXt-50~\cite{hu2018squeeze} & 78.9 & 94.5 & 4233 & 27.6 & - & - & -\\
		SKNet-50~\cite{li2019selective} & 79.2 & - & 4470 & 27.5 & - & - & -\\
		SE-ResNet-50$^*$~\cite{hu2018squeeze} & 80.5 & 94.8 & 4094 & 30.6 & - & -\\
		\textbf{GreedyNASv2-L} & \textbf{81.1} & 95.4 & 4098 & 26.9 & 57 & 9 & 500\\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	\vspace{-2mm}
	%\end{center}
\end{table*}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/tables/merge_ops.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/sim.pdf}
    \makeatletter\def\@captype{figure}\makeatother
    \vspace{-2mm}
    \caption{Visualization of learned operation similarities at the 1st searching layer of MB-SE supernet.}
    \label{fig:sim}
    
    \centering
    \setlength\tabcolsep{2.2mm}
    \renewcommand\arraystretch{1.1}
    \footnotesize
    \makeatletter\def\@captype{table}\makeatother
    \caption{Summary of merged operations (partial) \wrt Figure~\ref{fig:sim}.}
    \begin{tabular}{ll|c|l}
		\Xhline{2\arrayrulewidth}
		\multicolumn{2}{c|}{Operation pair} & Similarity & Retained operation \\
		\hline
		MB3\_K7\_SE & MB6\_K7 & 0.95 & MB3\_K7\_SE\\
		MB3\_K7 & MB3\_K7\_SE & 0.89 & MB3\_K7\\
		MB3\_K3\_SE & MB6\_K5\_SE & 0.89 & MB3\_K3\_SE\\
		MB3\_K7 & MB6\_K7\_SE & 0.88 & MB3\_K7\\
		MB3\_K7 & MB6\_K7 & 0.87 & MB3\_K7\\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	\vspace{-2mm}
    \label{tab:merge_ops}
\end{figure}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/tables/nas_benchmark.tex <==
\begin{table}[t]
	\renewcommand\arraystretch{1.1}
	\setlength\tabcolsep{1.mm}
	\centering
	%\begin{center}
	\caption{Performance of our PU learning method compared with PN learning on NAS-Bench-Macro~\cite{su2021prioritized}.}
	\vspace{-2mm}
	\label{tab:nasbench}
	\footnotesize
	%\normalsize
	\begin{tabular}{c|cc|cc|cc|cc}
		\Xhline{2\arrayrulewidth}
		\multirow{2}*{Method} & \multicolumn{2}{c|}{1\% data} & \multicolumn{2}{c|}{10\% data} & \multicolumn{2}{c|}{50\% data} & \multicolumn{2}{c}{100\% data}\\
		\cline{2-9}
		~ & Pre. & Recall & Pre. & Recall & Pre. & Recall & Pre. & Recall\\
		\hline
		PU & 97.21 & 97.08 & 98.37 & 98.34 & 98.30 & 98.19 & 98.81 & 98.62\\
		PN & 79.52 & 85.82 & 78.74 & 93.14 & 88.45 & 85.21 & 85.55 & 90.24\\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	%\end{center}
\end{table}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/tables/nas_comparison.tex <==
\begin{table}[t]
	\renewcommand\arraystretch{1.1}
	\setlength\tabcolsep{1.17mm}
	\centering
	%\begin{center}
	\caption{Comparisons with our baseline methods on different scales of search spaces. Search spaces \textit{small}, \textit{medium}, and \textit{large} represent \textit{MB-SE}, \textit{MB-SE+MixConv}, and \textit{MB-SE+MixConv+Shuffle} in Table~\ref{tab:search_space}, respectively.}
	\vspace{-2mm}
	\label{tab:nas_comparison}
	\footnotesize
	%\normalsize
	\begin{tabular}{c|ccc|ccc}
		\Xhline{2\arrayrulewidth}
		\multirow{2}*{Method} & \multicolumn{3}{c|}{ACC (\%)} & \multicolumn{3}{c}{ACC on supernet (\%)}\\
		\cline{2-7}
		~ & small & medium & large & small & medium & large\\
		\hline
		SPOS~\cite{guo2020single} & 76.8 & 76.6 & 75.5 & 56.5 & 48.2 & 33.4\\
		GreedyNAS~\cite{you2020greedynas} & 77.1 & 76.8 & 76.5 & 57.6 & 49.3 & 35.1\\
		GreedyNASv2 & \textbf{77.3} & \textbf{77.4} & \textbf{77.5} & \textbf{58.1} & \textbf{55.5} & \textbf{43.8}\\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	\vspace{-2mm}
	%\end{center}
\end{table}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/tables/search_space.tex <==
\begin{table*}[t]
	\renewcommand\arraystretch{1.3}
	\setlength\tabcolsep{1.6mm}
	\centering
	%\begin{center}
	\caption{Summary of our search spaces. Details can be found in Supplementary Materials.}
	\vspace{-2mm}
	\label{tab:search_space}
	\footnotesize
	%\normalsize
	\begin{tabular}{l|c|c|c|l}
		\Xhline{2\arrayrulewidth}
		Search space & Size & \#Layers & \#Operations & Operations \\
		\hline
		MB-SE & $13^{21}\approx2\times10^{23}$ & 21 & 13 & \{ MB3, MB6 \} $\times$ \{ K3, K5, K7, K3\_SE, K5\_SE, K7\_SE \} + \{ ID \} \\
		%\hline
		MB-SE+MixConv & $17^{21}\approx7\times10^{25}$ & 21 & 17 & MB-SE $\cup$ \{ MB3\_MIX, MB6\_MIX, MB3\_MIX\_SE, MB6\_MIX\_SE \}\\
		%\hline
		MB-SE+MixConv+Shuffle & $21^{21}\approx6\times10^{27}$ & 21 & 21 & MB-SE+MixConv $\cup$ \{ Shuffle\_3, Shuffle\_5, Shuffle\_7, Shuffle\_x \}\\
		\hline
		Res-50-SE & $19^{16}\approx3\times10^{20}$ & 16 & 19 & \{ ResNet, ResNeXt \} $\times$ \{ K3, K5, K7 \} $\times$ \{ 0.5$\times$, 1$\times$, 1.5$\times$ \} + \{ ID \} \\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	\vspace{-2mm}
	%\end{center}
\end{table*}

==> GreedyNASv2_ Greedier Search with Greedy Path Filter/theorem1.tex <==
\newtheorem{theorem}{Theorem}
\begin{theorem}[multi-path sampling \cite{you2020greedynas}] \label{theorem1}
If $m$ paths are sampled uniformly i.i.d from $\A$, and the proportion of good paths in the search space is $p$, then it holds that at least $k(k\le m)$ paths are good paths with confidence
\begin{equation}
  \mathbb{P} :=   \sum_{j=k}^m\mathbb{C}_m^j p^j (1-p)^{m-j} .
\end{equation}
\end{theorem}
